Experimental emulation for OTFS waveform RF-impairments

Orthogonal time-frequency space (OTFS) waveform exceeds the challenges that face orthogonal frequency division multiplexing (OFDM) in the high-mobility environment with high time-frequency dispersive channels. Since practical pulse shaping design and RF-impairments effects have a direct impact on waveform behavior, this paper investigates experimental implementation for practical pulse shaping design and RF-impairments that affect OTFS waveform performance and compares them to OFDM waveform as a benchmark. Firstly, the doubly-dispersive channel effect is analyzed, then an experimental framework is established for investigating the RF-impairments include non-linearity, Carrier frequency offset, I/Q-imbalances, DC-offset, and phase noise are considered. The experiments were conducted in a real indoor wireless environment using software-defined radio (SDR)based on the Keysight EXG X-Serie devices. The experimental results validate the accuracy of the theoretical results.

==> Experimental emulation for OTFS waveform RF-impermeant Access final work/acro.tex <==
\DeclareAcronym{RIS}{
  short = RIS ,
  long  = reconfigurable intelligent surfaces ,
  class = abbrev
}
\DeclareAcronym{6G}{
  short = 6G,
  long  = sixth generation ,
  class = abbrev
}
\DeclareAcronym{5G}{
  short = 5G,
  long  = fifth generation ,
  class = abbrev
}
\DeclareAcronym{EM}{
  short = EM ,
  long  = electromagnetic,
  class = abbrev
}
\DeclareAcronym{BS}{
  short = BS,
  long  = base station ,
  class = abbrev
}
\DeclareAcronym{UE}{
  short = UE ,
  long  = user equipment ,
  class = abbrev
}
\DeclareAcronym{MISO}{
  short = MISO,
  long  = multiple-input single-output ,
  class = abbrev
}
\DeclareAcronym{MMSE}{
  short = MMSE ,
  long  = minimum mean squared error ,
  class = abbrev
}
\DeclareAcronym{DFT}{
  short = DFT,
  long  = discrete Fourier transform ,
  class = abbrev
}
\DeclareAcronym{THz}{
  short = THz,
  long  = Terahertz ,
  class = abbrev
}
\DeclareAcronym{IoT}{
  short = IoT,
  long  = internet of things ,
  class = abbrev
}
\DeclareAcronym{MSE}{
  short = MSE,
  long  = mean square error ,
  class = abbrev
}
\DeclareAcronym{CSI}{
  short = CSI ,
  long  = channel state information ,
  class = abbrev
}
\DeclareAcronym{MIMO}{
  short = MIMO,
  long  = multiple-input multiple-output ,
  class = abbrev
}
\DeclareAcronym{UPA}{
  short = UPA,
  long  = uniform planner array ,
  class = abbrev
}
\DeclareAcronym{RF}{
  short = RF,
  long  = radio-frequency ,
  class = abbrev
}
\DeclareAcronym{mmWave}{
  short = mmWave,
  long  = millimeter-wave ,
  class = abbrev
}
\DeclareAcronym{AoA}{
  short = AoA ,
  long  = angle of arrival ,
  class = abbrev
}
\DeclareAcronym{AoD}{
  short = AoD,
  long  = angle of departure ,
  class = abbrev
}
\DeclareAcronym{EKF}{
  short = EKF,
  long  = extended Kalman filter ,
  class = abbrev
}
\DeclareAcronym{LMS}{
  short = LMS,
  long  = least mean square ,
  class = abbrev
}
\DeclareAcronym{BiLMS}{
  short = BiLMS,
  long  = bi-directional LMS ,
  class = abbrev
}
\DeclareAcronym{SNR}{
  short = SNR,
  long  = signal-to-noise ratio ,
  class = abbrev
}
\DeclareAcronym{LoS}{
  short = LoS,
  long  = line-of-sight ,
  class = abbrev
}
\DeclareAcronym{TDD}{
  short = TDD,
  long  = time-division duplexing ,
  class = abbrev
}
\DeclareAcronym{NMSE}{
  short = NMSE,
  long  = normalized mean square error ,
  class = abbrev
}
\DeclareAcronym{SDR}{
  short = SDR,
  long  = semidefinite relaxation ,
  class = abbrev
}
\DeclareAcronym{QoS}{
  short = QoS,
  long  = quality of service ,
  class = abbrev
}
\DeclareAcronym{NOMA}{
  short = NOMA,
  long  = non-orthogonal multiple access ,
  class = abbrev
}
\DeclareAcronym{OFDM}{
  short = OFDM,
  long  = orthogonal frequency division multiplexing ,
  class = abbrev
}
\DeclareAcronym{OMA}{
  short = OMA,
  long  = orthogonal multiple access ,
  class = abbrev
}
\DeclareAcronym{NU}{
  short = NU,
  long  = near user ,
  class = abbrev
}
\DeclareAcronym{FU}{
  short = FU,
  long  = far user ,
  class = abbrev
}
\DeclareAcronym{SIC}{
  short = SIC,
  long  = successive interference cancellation ,
  class = abbrev
}
\DeclareAcronym{PLS}{
  short = PLS,
  long  = physical layer security ,
  class = abbrev
}
\DeclareAcronym{MRT}{
  short = MRT,
  long  = maximum ratio transmission ,
  class = abbrev
}
\DeclareAcronym{AWGN}{
  short = AWGN,
  long  = additive white Gaussian noise,
  class = abbrev
}
\DeclareAcronym{SINR}{
  short = SINR,
  long  = signal-to-interference-plus-noise ratio ,
  class = abbrev
}
\DeclareAcronym{BPSK}{
  short = BPSK,
  long  = binary phase shift keying ,
  class = abbrev
}
\DeclareAcronym{QPSK}{
  short = QPSK,
  long  = quadrature phase shift keying ,
  class = abbrev
}
\DeclareAcronym{SVD}{
  short = SVD,
  long  = singular value decomposition ,
  class = abbrev
}
\DeclareAcronym{EVD}{
  short = EVD,
  long  = eigenvalue decomposition ,
  class = abbrev
}
\DeclareAcronym{PDF}{
  short = PDF,
  long  = probability density function ,
  class = abbrev
}
\DeclareAcronym{SER}{
  short = SER,
  long  = symbol error rate ,
  class = abbrev
}
\DeclareAcronym{MGF}{
  short = MGF,
  long  = moment generating function ,
  class = abbrev
}
\DeclareAcronym{2D}{
  short = 2D,
  long  = two-dimensional ,
  class = abbrev
}
\DeclareAcronym{3D}{
  short = 3D,
  long  = three-dimensional ,
  class = abbrev
}
\DeclareAcronym{CLT}{
  short = CLT,
  long  = central limit theorem ,
  class = abbrev
}
\DeclareAcronym{QAM}{
  short = QAM,
  long  = quadrature amplitude modulation ,
  class = abbrev
}
\DeclareAcronym{SISO}{
  short = SISO,
  long  = single-input single-output ,
  class = abbrev
}
\DeclareAcronym{CE}{
  short = CE,
  long  = channel estimation ,
  class = abbrev
}
\DeclareAcronym{KG}{
  short = $K_G$,
  long  = generalized-K ,
  class = abbrev
}
\DeclareAcronym{LSKRF}{
  short = LSKRF,
  long  = least squares Khatri-Rao factorization ,
  class = abbrev
}
\DeclareAcronym{IFFT}{
  short = IFFT,
  long  = inverse fast Fourier transform ,
  class = abbrev
}
\DeclareAcronym{FFT}{
  short = FFT,
  long  = fast Fourier transform ,
  class = abbrev
}
\DeclareAcronym{CP}{
  short = CP,
  long  = cyclic prefix ,
  class = abbrev
}
\DeclareAcronym{ISI}{
  short = ISI,
  long  = inter-symbol interference ,
  class = abbrev
}
\DeclareAcronym{CIR}{
  short = CIR,
  long  = channel impulse response ,
  class = abbrev
}
\DeclareAcronym{LS}{
  short = least square,
  long  = channel impulse response ,
  class = abbrev
}
\DeclareAcronym{CFR}{
  short = CFR,
  long  = channel frequency response ,
  class = abbrev
}
\DeclareAcronym{OTFS}{
  short = OTFS,
  long  = orthogonal time frequency space ,
  class = abbrev
}
\DeclareAcronym{BER}{
  short = BER,
  long  = bit error rate ,
  class = abbrev
} 
\DeclareAcronym{PAPR}{
  short = PAPR,
  long  = peak-to-average power ratio ,
  class = abbrev
}
\DeclareAcronym{GFDM}{
  short = GFDM,
  long  = generalized frequency division multiplexing ,
  class = abbrev
}
\DeclareAcronym{CFO}{
  short = CFO,
  long  = carrier frequency offset ,
  class = abbrev
}
\DeclareAcronym{CCDF}{
  short = CCDF,
  long  =complementary cumulative distribution function ,
  class = abbrev
}
\DeclareAcronym{ICI}{
  short = ICI,
  long  = intercarrier-interference ,
  class = abbrev
}

\DeclareAcronym{VSA}{
  short = VSA,
  long  = vector signal analyzer,
  class = abbrev
}




